The Submodular Santa Claus Problem in the Restricted Assignment Case

The submodular Santa Claus problem was introduced in a seminal work by Goemans, Harvey, Iwata, and Mirrokni (SODA'09) as an application of their structural result. In the mentioned problem $n$ unsplittable resources have to be assigned to $m$ players, each with a monotone submodular utility function $f_i$. The goal is to maximize $\min_i f_i(S_i)$ where $S_1,\dotsc,S_m$ is a partition of the resources. The result by Goemans et al. implies a polynomial time $O(n^{1/2 +\varepsilon})$-approximation algorithm. Since then progress on this problem was limited to the linear case, that is, all $f_i$ are linear functions. In particular, a line of research has shown that there is a polynomial time constant approximation algorithm for linear valuation functions in the restricted assignment case. This is the special case where each player is given a set of desired resources $\Gamma_i$ and the individual valuation functions are defined as $f_i(S) = f(S \cap \Gamma_i)$ for a global linear function $f$. This can also be interpreted as maximizing $\min_i f(S_i)$ with additional assignment restrictions, i.e., resources can only be assigned to certain players. In this paper we make comparable progress for the submodular variant. Namely, if $f$ is a monotone submodular function, we can in polynomial time compute an $O(\log\log(n))$-approximate solution.

==> submodular.tex <==
A prominent case of the Santa Claus problem is the restricted Santa Claus problem where all valuations of resources we have $v_{ij}\in \{0,v_j\}$. In this case, it is known how to obtain a constant factor approximation. The problem can be rewritten as follows. Define a linear function $f: S\subseteq R\mapsto \mathbb R$ where $f(S)=\sum_{j\in S}v_j$ and a subset $R_i\subseteq R$ for every player $i$. Then the restricted Santa Claus problem can be formulated as finding a partition $S_1,S_2,\ldots , S_m$ of the resource set such that 
\begin{equation*}
    \min_{i\in P} f(S_i\cap R_i)
\end{equation*} is maximized. A very natural extension of this problem is to consider $f$ as non necessarily linear. For instance, $f$ can be submodular. We show that our result also implies a $O(\log \log (|R|))$-approximation when $f$ is submodular.
